Comet: Fine-grained Computation-communication Overlapping for Mixture-of-Experts

Mixture-of-experts (MoE) has been extensively employed to scale large language models to trillion-plus parameters while maintaining a fixed computational cost. The development of large MoE models in the distributed scenario encounters the problem of large communication overhead. The inter-device communication of a MoE layer can occupy 47% time of the entire model execution with popular models and frameworks. Therefore, existing methods suggest the communication in a MoE layer to be pipelined with the computation for overlapping. However, these coarse grained overlapping schemes introduce a notable impairment of computational efficiency and the latency concealing is sub-optimal. To this end, we present COMET, an optimized MoE system with fine-grained communication-computation overlapping. Leveraging data dependency analysis and task rescheduling, COMET achieves precise fine-grained overlapping of communication and computation. Through adaptive workload assignment, COMET effectively eliminates fine-grained communication bottlenecks and enhances its adaptability across various scenarios. Our evaluation shows that COMET accelerates the execution of a single MoE layer by $1.96\times$ and for end-to-end execution, COMET delivers a $1.71\times$ speedup on average. COMET has been adopted in the production environment of clusters with ten-thousand-scale of GPUs, achieving savings of millions of GPU hours.

==> sections/moti_znx.tex <==
\section{Background and motivation}
Mixture of Experts (MoE) is key to efficiently scaling models. By sparsely activating different experts, MoE allows models to incorporate more parameters without increasing inference costs, leading to improved performance. This is particularly important in the era of large models. Notably, with the discovery in GPT-4-o1 that scaling inference time can further enhance model capabilities, MoE’s inherent advantage in inference efficiency positions it as a critical component in the era of large-scale models.

\subsection{Joint optimization of computation and communication }
show that optimization the communication in the MoE is critical, can also breifly describe the parallism method in MoE (EP, TP)

\subsection{Mismatch in the granularity of computation and communication}

\paragraph{Complex data dependency}

\paragraph{Finegrained communication I/O}
